SquirrelFS: using the Rust compiler to check file-system crash consistency

This work introduces a new approach to building crash-safe file systems for persistent memory. We exploit the fact that Rust's typestate pattern allows compile-time enforcement of a specific order of operations. We introduce a novel crash-consistency mechanism, Synchronous Soft Updates, that boils down crash safety to enforcing ordering among updates to file-system metadata. We employ this approach to build SquirrelFS, a new file system with crash-consistency guarantees that are checked at compile time. SquirrelFS avoids the need for separate proofs, instead incorporating correctness guarantees into the typestate itself. Compiling SquirrelFS only takes tens of seconds; successful compilation indicates crash consistency, while an error provides a starting point for fixing the bug. We evaluate SquirrelFS against state of the art file systems such as NOVA and WineFS, and find that SquirrelFS achieves similar or better performance on a wide range of benchmarks and applications.

==> sections/figures/intro_typestate_diagram.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.35]{sections/figures/intro_typestate_diagram.png}
    \caption{A comparison of type representations of a persistent inode structure as operations modify the inode. With an initialization operation, the inode goes from free (white) to initialized (gray), but it is still dirty (fine dotted outline); multiple persistence primitives must be used to ensure it becomes persistent. In a standard, non-typestate based file system, the inode's type remains the same throughout all of these operations; developers must remember (or check at runtime) whether the inode has been fully initialized and include proper persistence operations. With typestate, both persistence and operational information is encoded into the inode's type and can be typechecked to ensure the inode is clean and initialized by the end of the operation.}
    \label{fig:intro_typestate}
\end{figure*}

==> sections/figures/typestate_listing.tex <==
\begin{lstlisting}[language=Rust,float,caption={
    Pseudocode example of several Rust structs with typestates as generic type parameters. Each method is only defined on objects with certain typestates.
},label=lst:typestate,captionpos=b] 
impl Inode<Free> {
    fn init_inode(self, ...)
        -> Inode<Init> {...}
}
impl Dentry<Free> {
    fn set_name(self, name: String)
        -> Dentry<Init> {...}
}
impl Dentry<Init> {
    fn commit_dentry(
        self, 
        inode: Inode<Init>
    ) -> Dentry<Committed> {..}
}
\end{lstlisting}





